Improving Automatic Parallel Training via Balanced Memory Workload Optimization

Transformer models have emerged as the leading approach for achieving state-of-the-art performance across various application domains, serving as the foundation for advanced large-scale deep learning (DL) models. However, efficiently training these models across multiple GPUs remains a complex challenge due to the abundance of parallelism options. Existing DL systems either require manual efforts to design distributed training plans or limit parallelism combinations to a constrained search space. In this paper, we present Galvatron-BMW, a novel system framework that integrates multiple prevalent parallelism dimensions and automatically identifies the most efficient hybrid parallelism strategy. To effectively navigate this vast search space, we employ a decision tree approach for decomposition and pruning based on intuitive insights. We further utilize a dynamic programming search algorithm to derive the optimal plan. Moreover, to improve resource utilization and enhance system efficiency, we propose a bi-objective optimization workflow that focuses on workload balance. Our evaluations on different Transformer models demonstrate the capabilities of Galvatron-BMW in automating distributed training under varying GPU memory constraints. Across all tested scenarios, Galvatron-BMW consistently achieves superior system throughput, surpassing previous approaches that rely on limited parallelism strategies.

==> plots/apis.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figure/apis.png}
    \caption{Comparsion between ordinary model training and Galvatron model training.}
    \label{fig:apis}
\end{figure}

==> plots/cost_estimation.tex <==
% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{figure/estimatedcost.png}
%     \label{fig:costestimation}
%     \caption{Accuracy of estimation with (left) and without (right) overlap coefficient. Different markers represent different models.}
%     \label{fig:Cost_estimation}
% \end{figure}

\begin{figure}[t]
\centering
%\subfigure[w. overlapping slowdown]{
\begin{minipage}[t]{0.48\linewidth}
%\scalebox{.46}{
\includegraphics[width=1.0\linewidth]{figure/estimatedcost_w.png}
%}
%\label{fig:worker_homo}
%}
\vspace{-6mm}
\subcaption{w. overlapping slowdown}
\end{minipage}
% \subfigure[w.o. overlapping slowdown]{
% \scalebox{.46}{
\begin{minipage}[t]{0.48\linewidth}
\includegraphics[width=1.0\linewidth]{figure/estimatedcost_wo.png}
% }
%\label{fig:worker_hete}
% }
\vspace{-6mm}
\subcaption{w.o. overlapping slowdown}
\end{minipage}
\vspace{-2mm}
\caption{Estimation errors with and without considering the overlapping slowdown.}\label{fig:costestimation}
\vspace{-6mm}
\end{figure}
